Dodo: Dynamic Contextual Compression for Decoder-only LMs

Transformer-based language models (LMs) are inefficient in long contexts. We propose Dodo, a solution for context compression. Instead of one vector per token in a standard transformer model, Dodo represents text with a dynamic number of hidden states at each layer, reducing the cost of self-attention to a fraction of typical time and space. Moreover, off-the-shelf models such as LLaMA can be adapted to Dodo by efficient parameter tuning methods such as LoRA. In use, Dodo can act as either an autoregressive LM or a context compressor for downstream tasks. We demonstrate through experiments in language modeling, question answering, and summarization that Dodo retains capabilities in these tasks, while drastically reducing the overhead during decoding. For example, in the autoencoding task, Dodo shrinks context at a 20x compression ratio with a BLEU score of 98% for reconstruction, achieving nearly lossless encoding.

==> 87straight_through.tex <==


\section{Training Scorer with straight-through estimator}
\label{app:residual_connection}

In \cref{sec:residual}, we propose to build a residual connection between nugget scores and the self-attention of the decoder transformers to back-propagate gradients to $\mathtt{Scorer}$.
We copy it here:
\begin{align}
    \xi_{i,j}^l = \frac{1}{\sqrt{d}}\left[\left( \vec{W}^\text{Q} \vec{x}_i^l\right)^\top\left(\vec{W}^\text{K}\vec{x}_j^l\right) {\color{red}+ s_j}\right],
    \quad i < j.
    \label{eq:copy_residual}
\end{align}

However, adding nugget scores to the attention logits affects the behavior of self-attention.
In practice, we found that the nugget score (i.e. $s_j$ in \cref{eq:copy_residual}) is of a similar scale of attention logits (i.e. $\left( \vec{W}^\text{Q} \vec{x}_i^l\right)^\top\left(\vec{W}^\text{K}\vec{x}_j^l\right)$ in \cref{eq:copy_residual}) and the nugget scores are usually positive, meaning that nugget tokens draw more attention because of the addition of $s_j$.

Alternatively, we propose to remove the effect of $s_j$ in \cref{eq:copy_residual} from the forward propagation of the neural network:
\begin{align}
    \xi_{i,j}^l = \frac{1}{\sqrt{d}}\left[\left( \vec{W}^\text{Q} \vec{x}_i^l\right)^\top\left(\vec{W}^\text{K}\vec{x}_j^l\right) {\color{red}+ s_j}{\color{blue} - \mathtt{StopGrad}(s_j)}\right],
    \quad i < j,
    \label{eq:straight_through}
\end{align}
where $\mathtt{StopGrad}$ means detaching it from the computation graph.
Therefore, $s_j$ receives the same gradients as the attention logits, but they do not impact the attention distribution.
This is akin to the ``straight-through estimator'' discussed in \citet{straightthrough13}.

In practice, the behavior of both \cref{eq:copy_residual,eq:straight_through} is similar: They quickly converge --- the nugget selection is stable after 3000 steps of training --- and they have similar performance on the autoencoding experiments in \cref{sec:autoencoding}.
One can even remove the residual connection in \cref{eq:copy_residual} when the $\mathtt{Scorer}$ converges (after 3000 steps of training) and the model can quickly adapt to the new attention pattern.
We speculate that Llama-7b permits more flexibility because of its tremendous size.


==> 90nugget.tex <==
\section{A detailed comparison between \textsc{Nugget} and \textsc{Nugget2D}}
\label{app:nugget}

In this section, we show more details on the architecture of \textsc{Nugget} and a succinct comparison between \textsc{Nugget} and \textsc{Nugget2D}.
While \citet{nugget23} provides a thorough discussion  of \textsc{Nugget}. %

\paragraph{Applicability}
\citet{nugget23} can be applied to the encoder-side of an encoder-decoder transformer and \nugget can be applied to decoder-only transformers, such as \textsc{LLaMA}.

\paragraph{The form of nuggets}
The decoder exclusively attends to the last-layer representation of the encoder side, thus each nugget in \citet{nugget23} is the last-layer representation of its corresponding token ($\vec{z}_i \in \mathbb{R}^{d}$).
For a decoder-only transformer, each future token attends to all-layer hidden states of past tokens. Therefore, a nugget in \model is comprised of the hidden states of the corresponding token in all the layers ($\vec{z}_i \in \mathbb{R}^{L \times d}$, $L$ is the number of layers).

\paragraph{The learning of nugget selection}
Both \citet{nugget23} and \model have a nugget selection module $\sco$. 
In \citet{nugget23}, $\sco$ takes features from the $l$-th layer of the transformer encoder, thus they freeze the first $l$ transformer layers to make the training stable.
In \model, $\sco$ takes features from a frozen transformer decoder with $l$ layers that are initialized from \textsc{LLaMA}, thus all the layers of the encoder ($\phi$) and decoder ($\theta$) are trainable.

Although \citet{nugget23} uses a transformer encoder to represent text, a dual decoder must be equipped during the training phase to learn the nugget selection module.
Suppose $\mathtt{Scorer}$ is used to select nuggets, which outputs a score $s_i \in \mathbb{R}$ for the $i$-th token, it is plugged into the \emph{cross-attention} to receive gradients:
\begin{align}
a_{i,j} = \frac{1}{\sqrt{d}} \left[ \left(\vec{W}^\text{Q}\vec{x}_j^\text{tgt}\right)^\top\left(\vec{W}^\text{K}\vec{z}_i\right) + s_i  \right], \nonumber
\end{align}
where $a_{i,j}$ is the attention score from the $j$-th token $\vec{x}^\text{tgt}_j$ on the target side to the $i$-th nugget $\vec{z}_i$.
Note that the auxiliary decoder of \citet{nugget23} is discarded after training.

In contrast, \model directly works on a transformer decoder, thus the training of the $\mathtt{Scorer}$ in \model is straightforward.
In \model, the residual connection between $\mathtt{Scorer}$ and the \emph{self-attention} is built to learn nuggets (refer to \cref{eq:residual}.
\model does not require an auxiliary module to learn nuggets.

\paragraph{Flexibility on text compression}
\citet{nugget23} compresses the entire text with a transformer encoder.
\model can compress any part of the text.
Similar to our experiments on \cref{sec:lm_exp,sec:qa}, one may flexibly choose to compress a certain part of the text.

\paragraph{Streaming decoding}
Due to the nature of the transformer encoder, \citet{nugget23} can only encode the text.
Its decoder can learn to decode new texts, but it cannot re-encode them to nuggets in an efficient way.
\model, with parameter re-assignment described in \cref{sec:asauto}, can naturally decode new texts and re-encode them auto-regressively, achieving streaming decoding.

\paragraph{Nugget type encoding}
\citet{nugget23} passes a ``type embedding'' during the encoding process to inform the model what tokens are selected as nuggets (eq 8 in their paper).
Empirically we do not find any improvement after introducing the ``type embedding'', thus our experiments in the main paper are conducted without type embeddings.
We speculate there are 2 reasons behind this:
\begin{enumerate}
    \item An encoder transformer may not naturally concentrate context information into a few tokens, as the cross-attention from the decoder side always covers all token representations.
    In this case, a type embedding can guide the model to encode context semantics in nugget tokens.
    However, during the pretraining phase of a decoder-only transformer, the embedding of each token is used to predict the next token, thus it naturally gathers context information.
    In this case, a type embedding is redundant.
    \item In the architecture of autoregressive \model in \cref{sec:asauto}, nugget tokens are encoded with parameter $\phi$ instead of $\theta$ that are used for non-nugget tokens.
    A separate type embedding to distinguish nugget tokens is obviously unnecessary in this case.
\end{enumerate}

